Speech Foundation Models and Crowdsourcing for Efficient, High-Quality Data Collection

While crowdsourcing is an established solution for facilitating and scaling the collection of speech data, the involvement of non-experts necessitates protocols to ensure final data quality. To reduce the costs of these essential controls, this paper investigates the use of Speech Foundation Models (SFMs) to automate the validation process, examining for the first time the cost/quality trade-off in data acquisition. Experiments conducted on French, German, and Korean data demonstrate that SFM-based validation has the potential to reduce reliance on human validation, resulting in an estimated cost saving of over 40.0% without degrading final data quality. These findings open new opportunities for more efficient, cost-effective, and scalable speech data acquisition.

==> images/diagram_application.tex <==
\begin{figure*}[ht]
    \centering
    \includegraphics[width=\textwidth,keepaspectratio]{images/diagram_application.png} 
    \caption{Overall processes differences. \textcolor{red}{Image to be replaced with better one in the later version}}
    \label{fig:application_diagram}
\end{figure*}

==> images/methods_flow.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.5\textwidth,keepaspectratio]{images/methods_flow.png} 
    \caption{Prescreen method differnces. \textcolor{red}{Image to be replaced with better one in the later version}}
    \label{fig:methods_flow}
\end{figure}

==> images/trade_off_graph_content.tex <==
\begin{figure}[ht]
    \centering
    \includesvg[width=0.5\textwidth,keepaspectratio]{images/trade_off_graph.svg} 
    \caption{Trade-off between validation cost and dataset quality}
    \label{fig:tradeoff_graph}
\end{figure}

==> sections/acknowledgments.tex <==
% This document has been adapted by Emily Allaway from the instructions for earlier ACL and NAACL proceedings, including those for NAACL 2024 by Steven Bethard, Ryan Cotterell and Rui Yan,
% ACL 2019 by Douwe Kiela and Ivan Vuli\'{c},
% NAACL 2019 by Stephanie Lukin and Alla Roskovskaya,
% ACL 2018 by Shay Cohen, Kevin Gimpel, and Wei Lu,
% NAACL 2018 by Margaret Mitchell and Stephanie Lukin,
% Bib\TeX{} suggestions for (NA)ACL 2017/2018 from Jason Eisner,
% ACL 2017 by Dan Gildea and Min-Yen Kan,
% NAACL 2017 by Margaret Mitchell,
% ACL 2012 by Maggie Li and Michael White,
% ACL 2010 by Jing-Shin Chang and Philipp Koehn,
% ACL 2008 by Johanna D. Moore, Simone Teufel, James Allan, and Sadaoki Furui,
% ACL 2005 by Hwee Tou Ng and Kemal Oflazer,
% ACL 2002 by Eugene Charniak and Dekang Lin,
% and earlier ACL and EACL formats written by several people, including
% John Chen, Henry S. Thompson and Donald Walker.
% Additional elements were taken from the formatting instructions of the \emph{International Joint Conference on Artificial Intelligence} and the \emph{Conference on Computer Vision and Pattern Recognition}.

==> sections/related_work.tex <==
\textcolor{red}{We limit the related work to be max 0.75 page.}
To produce a PDF file, pdf\LaTeX{} is strongly recommended (over original \LaTeX{} plus dvips+ps2pdf or dvipdf). Xe\LaTeX{} also produces PDF files, and is especially suitable for text in non-Latin scripts.

==> tables/decision_tree_w_silver.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c|c|c|c|c|c|c|}
\cline{2-7}
 &
  \textbf{Features} &
  \textbf{Precision} &
  \textbf{Recall} &
  \textbf{\begin{tabular}[c]{@{}c@{}}F1\\ score\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Type 1\\ error\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Type 2\\ error\end{tabular}} \\ \hline
\multicolumn{1}{|c|}{DW 1+S} & DW 1 + silver & 0.674 & 0.512 & 0.582 & 0.011 & 0.488 \\ \hline
\multicolumn{1}{|c|}{DW 2+S} & DW 2 + silver & 0.619 & 0.520 & 0.565 & 0.014 & 0.480 \\ \hline
\multicolumn{1}{|c|}{DW 3+S} & DW 3 + silver & 0.631 & 0.520 & 0.570 & 0.013 & 0.480 \\ \hline
\multicolumn{1}{|c|}{DW 4+S} & DW 4 + silver & 0.730 & 0.432 & 0.543 & 0.007 & 0.568 \\ \hline
\multicolumn{1}{|c|}{DW 5+S} & DW 5 + silver & 0.569 & 0.528 & 0.548 & 0.018 & 0.472 \\ \hline
\multicolumn{1}{|c|}{DW 6+S} & DW 6 + silver & 0.681 & 0.512 & 0.584 & 0.011 & 0.488 \\ \hline
\multicolumn{1}{|c|}{DW 7+S} & DW 7 + silver & 0.681 & 0.512 & 0.584 & 0.011 & 0.488 \\ \hline
\end{tabular}%
}
\caption{Decision tree performance with adding silver label in the feature set.\textcolor{red}{to be removed if Figure 1 looks good.}}
\label{tab:decision_tree_w_silver}
\end{table}

==> tables/decision_tree_wo_silver.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|l|c|c|c|c|c|}
\cline{2-7}
 &
  \textbf{Features} &
  \textbf{Precision} &
  \textbf{Recall} &
  \textbf{\begin{tabular}[c]{@{}c@{}}F1\\ score\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Type 1\\ error\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Type 2\\ error\end{tabular}} \\ \hline
\multicolumn{1}{|l|}{DW 1} & WER          & 0.096 & 0.072 & 0.082 & 0.030 & 0.928 \\ \hline
\multicolumn{1}{|l|}{DW 2} & CER          & 0.387 & 0.096 & 0.154 & 0.007 & 0.904 \\ \hline
\multicolumn{1}{|l|}{DW 3} & PER          & 0.435 & 0.080 & 0.135 & 0.005 & 0.920 \\ \hline
\multicolumn{1}{|l|}{DW 4} & TER          & 0.081 & 0.600 & 0.143 & 0.299 & 0.400 \\ \hline
\multicolumn{1}{|l|}{DW 5} & DT-W 1 + CER & 0.387 & 0.096 & 0.154 & 0.007 & 0.904 \\ \hline
\multicolumn{1}{|l|}{DW 6} & DT-W 5 + PER & 0.440 & 0.088 & 0.147 & 0.005 & 0.912 \\ \hline
\multicolumn{1}{|l|}{DW 7} & DT-W 6 + TER & 0.387 & 0.096 & 0.154 & 0.007 & 0.904 \\ \hline
\end{tabular}%
}
\caption{Decision tree performance.\textcolor{red}{to be removed if Figure 1 looks good.}}
\label{tab:decision_tree}
\end{table}

==> tables/simple_policy.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[hbt!]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|l|c|c|c|c|c|}
\hline
 &
  Precision &
  Recall &
  \begin{tabular}[c]{@{}c@{}}F1\\ Score\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Type 1\\ error\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Type 2\\ error\end{tabular} \\ \hline
CER\&WER == 0 &
  0.072 &
  0.936 &
  0.134 &
  0.530 &
  0.064 \\ \hline
\end{tabular}%
}
\caption{Distance-based automated validation result on test split. \textcolor{red}{to be moved to the Appendix \ref{apdx:metric_comparison} if the space is limited.}}
\label{tab:simple_policy}
\end{table}
